Robust cross-domain disfluency detection with pattern match networks

In this paper we introduce a novel pattern match neural network architecture that uses neighbor similarity scores as features, eliminating the need for feature engineering in a disfluency detection task. We evaluate the approach in disfluency detection for four different speech genres, showing that the approach is as effective as hand-engineered pattern match features when used on in-domain data and achieves superior performance in cross-domain scenarios.

==> analysis.tex <==
The difficulty in applying the model on out-of-domain data lie in both difference in corpora and underlying model. There is substantial variation in vocabulary, conversational style, disfluency types, and sentence segmentation criteria across corpora. CallHome is more casual than SWBD; SCOTUS and FCIC are formal high stakes discussions with vocabularies highly dissimilar to SWBD. SCOTUS, FCIC, and CallHome contain 2, 5 and 7 times more restarts token-wise, respectively, than Switchboard. Also, on average, disfluencies in all three out-of-the-domain corpora tend to be longer, especially in CallHome and FCIC. 


\begin{table} [t]
\begin{center}
\begin{tabular}{|l|l|c|c|c|}
\hline \multicolumn{2}{|c|}{} & CallHome &  SCOTUS & FCIC\\ \hline
\multirow{3}{*}{\bf Model (Prec)}& CRF  & 71.5 & 90.9 & 88.7 \\
& LSTM  & 54.7 & 71.8 & 58.7 \\
& LSTM pm net  & 68.4 & 88.0 & 87.2 \\ \hline
\multirow{2}{*}{\bf Statistics} & OOV in disfl & 3\% & 6.4\% & 7.6\% \\
& Repetitions & 30.2\% & 59.5\% & 28.5\% \\ \hline
\end{tabular}
\end{center}
\caption{\label{tab:oov} \textbf{Top:} Precision scores for CRF, LSTM with hand-engineered pattern match features and LSTM with PMN. \textbf{Bottom:}Statistics on percentage of OOV words that are part of disfluency (< 10 words in training set) and percentage of tokens in disfluencies that are repetitions.}
\end{table}


\begin{table} [t]
\begin{center}
\begin{tabular}{|l|c|c|c|c|}
\hline \bf Model & SWBD dev & CallHome &  SCOTUS & FCIC\\ \hline
CRF  & 8.2 & 23.6 & 20.7 & 17.2 \\ \hline
LSTM  & 0.8 & 2.7 & 1.6 & 2.9 \\ \hline
LSTM pm net & 70.7 & 45.4 & 65.9 & 39\\ \hline
\end{tabular}
\end{center}
\caption{\label{tab:unk} F1 scores for CRF, LSTM with hand-engineered pattern match features and LSTM with PMN when tested on a text with tokens replaced by "UNK".}
\end{table}

\subsection{Model analysis}
In order to better understand the differences of the models that rely on pattern match features (hand-crafted or automatic), we perform the following ablation experiment. We substitute all token identities in our test data for each of the domain with general "UNK" token used for all out-of-vocabulary (OOV) words, thus relying most of predict power on pattern match features. For PMN, we keep the token identity only to calculate similarity features, but then substitute it with "UNK" for the rest of the model. We apply models trained on the regular data and used in Table \ref{tab:results} in order to evaluate how good the model can perform when all the tokens are OOVs. F1 scores are shown in Table \ref{tab:unk}. From the results we can see that LSTM with PMN is highly relies on the learned pattern match features, while LSTM with hand-crafted features almost fully relying on token identities. This might explain a very poor performance of LSTM with hand-crafted features in out-of-domain experiments, where there there is a big vocabulary and style differences. On the other hand, CRF serves as a solid baseline, and substantially relies on hand-crafted features comparing to LSTM. 

By looking at the precision vs. recall of the models we noticed that the main drop in performance in LSTM with hand-derived features comes low precision (Table \ref{tab:oov}). In particular, the LSTM with pattern match features ``hallucinates" a lot of disfluencies, longer ones in particular.
On the other hand if we look at the relative drop in performance between LSTMs with PMN vs. hand-crafted features, we can see that the relative difference in precision in CallHome and SCOTUS is similar, while FCIC is the most affected by the domain shift. SCOTUS and FCIC are two domains that are most affected by higher rates of OOVs in disfluencies (here defined as words that occur less than 10 times in the training set). While the OOV rates for FCIC and SCOTUS are similar, the drop in performance on SCOTUS is smaller, which can be explained by a higher number of repetitions which often are easier to predict.


\subsection{Error analysis}

\begin{table*}
\begin{center}
{\small
\begin{tabular}{|l|c|p{5.5in}|}\hline
\bf Corpus & \bf Ex & \bf Sentence\\ \hline
\multirow{2}{*}{CallHome} & 1 & Oh he [ looks like + John Travolta but he has like ] curly blond hair. \\
         & 2 & [ I do n't think + [ I know her + but I 've ] ] heard of her \\ \hline
         %& I do n't think we 're going [I hope not + I mean I 'd] like it under other circumstances but \dots \\ \hline
\multirow{2}{*}{SCOTUS}   & 3 & What is your [ authority + for that proposition, Mr. Guttentag, your case authority ] ? \\
         & 4 & \dots as to permit review in [ the court + of appeals, then the district court ] habeas corpus procedure need \dots \\ \hline
\multirow{2}{*}{FCIC}     & 5 &Thank you for the opportunity [ to + contribute to the commission 's work to ] understand the causes of \dots\\ 
         & 6 & \dots counter parties were unaware [ of + the full extent of ] those vehicles and therefore could not \dots \\ \hline
\end{tabular}
}
\end{center}
\caption{Example sentences wrongly predicted as disfluent by LSTM model with hand-crafted pattern match features. The brackets indicate predicted disfluency regions, where the respected gold annotation is ``non-disfluent". 
\label{tab:examples}}
\end{table*}

To confirm our conclusions, we look at examples of sentences (Table \ref{tab:examples}) with false positives made by the LSTM with hand-engineered features, but were correctly identify by our model. Those examples are consistent with the results that LSTM with hand-crafted features has a significant drop in precision.

%Table \ref{tab:oov} shows that that there is a significant drop in precision for LSTMs with hand-derived features. In particular, the LSTM with pattern match features ``hallucinates" a lot of disfluencies, longer ones in particular. %This might be due to the long memory of the LSTM, as opposed to CRF, which tends to be more local. %On the other hand, LSTM with our proposed pattern match architecture does not have much of false positives and behaves more similar to CRF rather than LSTM on out-of-the-domain data.
%Table \ref{tab:examples} presents some examples with false positives made by the LSTM with hand-engineered features, but were correctly identify by our model. 

%\begin{table} [t]
%\begin{center}
%\begin{tabular}{|l|c|c|c|c|c|c|}
%\hline  & \multicolumn{2}{c|}{CRF} &  \multicolumn{2}{c|}{LSTM} & \multicolumn{2}{c|}{LSTM sim}\\ 
%\hline \bf Corpus  & Prec & Rec & Prec & Rec & & \\ \hline \hline
%CallHome & 71.5 & 56.7 & 54.75 & 63.7 & &\\ \hline
%SCOTUS & 90.9 & 70.2 & 71.75 & 63.6 & &\\ \hline
%FCIC & 88.7 & 49.8 & 58.7 & 42.8 & &\\ \hline
%\end{tabular}
%\end{center}
%\caption{\label{tab:prec_rec} Not sure if we need this table, but just in case some results are useful. Precision and recall across domains for CRF and LSTM models when both identity and pattern match features used.}
%\end{table}


==> swbd.tex <==
\subsection{Transcription accuracy}

\subsection{Tokenization}

==> transformer.tex <==
In this section we want to make a more explicit comparison of our approach and some prior work that resembles some architectural similarity to our approach, and emphasize the novelty of the proposed architecture.

The Transformer \cite{vaswani2017attention} was first introduced in context of neural machine translation with encoder-decoder architecture. The main idea of the Transofrmer was to replace computationally costly RNNs and CNNs with multi-head self-attention mechanism at each layer.
As a result, 
The architecture fully relies on attention mechanism to learn global cross-token dependencies by learning to attend to any of the inputs from the previous (lower) layer. Later, \cite{shen2017disan} extended the Transformer for sentence-embedding task %without encoder-decoder architecture and 
with directional self-attention, using separate attention for forward and backward window. In our work, in order to learn pattern match features, we rely on multi-dimentional (akin multi-head in self-attention) similarity scores instead of attention scores, which we empirically found to work better in disfluency detection task. In addition, motivated by the fact that the repair always comes after the reparandum (meaning the physical proximity between the reparandum and repair tokens), we calculate similarity scores only in a limited size window, which removes unnecessary noise in longer sentences. .Nevertheless, our main difference to the prior work and novelty of this paper is in a usage of calculated similarity scores as features for CNN in order to find higher-order k-gram similarity pattern in a sentence (Section \ref{sec: conv_over_sim}). Unlike Transformer, we use LSTM on top for direct comparison of hand-crafted vs automatic pattern match features.

\begin{figure*}[t]
\includegraphics[scale=0.37]{att_net_cut.png}
\centering
\caption{An illustration of the model. In this example, the backward neighbor-similarity layer $\alpha^b$ identifies that \textit{``we"} has high similarity with \textit{``I"} and \textit{``were"} has high similarity with \textit{``was"}. Both \textit{``we"} and \textit{``were"} are at a distance of 3 from the corresponding \textit{``I"} and \textit{``was"}. A convolutional filter can catch the horizontal pattern in row 3, thus indicating the presence of a bigram pattern match between \textit{``we were"} and \textit{``I was"}. }%In this scheme $n=10$, $w=4$, $d_t+d_p=3$, $d_f=3$, 3 filter sizes: $[5,3],[5,1]$ and $[3,1]$, $l=1$ and $m=4$. }
\label{fig:model}
\end{figure*}



